Listen, Interact and Talk: Learning to Speak via Interaction

One of the long-term goals of artificial intelligence is to build an agent that can communicate intelligently with human in natural language. Most existing work on natural language learning relies heavily on training over a pre-collected dataset with annotated labels, leading to an agent that essentially captures the statistics of the fixed external training data. As the training data is essentially a static snapshot representation of the knowledge from the annotator, the agent trained this way is limited in adaptiveness and generalization of its behavior. Moreover, this is very different from the language learning process of humans, where language is acquired during communication by taking speaking action and learning from the consequences of speaking action in an interactive manner. This paper presents an interactive setting for grounded natural language learning, where an agent learns natural language by interacting with a teacher and learning from feedback, thus learning and improving language skills while taking part in the conversation. To achieve this goal, we propose a model which incorporates both imitation and reinforcement by leveraging jointly sentence and reward feedbacks from the teacher. Experiments are conducted to validate the effectiveness of the proposed approach.

==> blog.tex <==

Baby-like language learning via interaction

by Haichao Zhang, Haonan Yu and Wei Xu


In the blog post we unveiled a few weeks ago, we showed our results on how to teach our baby agent to understand the command from teacher and navigate in a maze accordingly.
Our AI agent has evolved since then with newly gained speaking capability. 

Our AI agents learns to speak in a way that is different from others. Conventional approaches rely on supervised training with large corpus of pre-collected training data, which typically requires a huge amount of human effort for collecting and annotating. More crucially, this is very different from how humans/babies learn.


%Humans act upon the world and learn from the consequences of their actions.
%For physical actions such as movement, the consequences mainly follow geometrical and mechanical principles, while for language, humans act by speaking and the consequence is typically response in the form of verbal and other behavioral feedbacks (\emph{e.g.}, nodding) from conversation partners. These feedbacks typically contain  informative signal on how to improve the language skills in  subsequent conversions and play an important role in human’s language acquisition process.
Our AI agents learning to speak by interacting with a virtual teacher/parent, just like a baby.
Baby interacts with people and learn through mimicking and feedbacks. 
For learning to speak, baby initially performs verbal action by mimicking his conversational parter (\emph{e.g.} parent) and masters the skill of generating a word (sentence). He could also possibly pick up the association of a word with a visual image when his parents saying ``\emph{this is apple}'' while pointing to an apple or an image of it.
Later, one can ask the baby question like ``\emph{what is this}'' while pointing to an  object, and provides the correct answer if the baby doesn't respond or responds incorrectly, which is typical in the initial stage.
One can also provide at the same time a verbal confirmation (\emph{e.g.} ``\emph{yes/no}'') with a nodding/smile/kiss/hug when he answers correctly as a form of encouragement feedback.
From a baby's perspective, the way to learn the language is by making verbal utterances to parent and adjusting his verbal behavior according to the corrections/confirmation/encouragement from parent. 
The language learning process of a baby is both impressive as a manifestation of human intelligence and inspiring for designing novel settings and algorithms for computational language learning.



Study Overview

This example illustrates that the language learning process is inherently  \emph{interactive}, a property which is potentially difficult to be captured by a static dataset as used in the conventional supervised learning setting.  
Inspired by baby's language learning process, we present a novel interactive setting for grounded natural language learning,  where the teacher and the learner can interact with each other in natural languages as shown in Figure~\ref{fig:example}. 
In this setting, there is no direct  supervisions to guide the behavior of the learner as in the  supervised learning setting. Instead, the 
learner has to \emph{act in order to learn}, \emph{i.e.},  engaging in the conversation with currently acquired speaking skills to obtain feedbacks from the dialogue partner, which provide learning signals for further improvement on the conversation skills. 

In this study, we propose a \emph{joint imitation and reinforcement} approach for interactive language learning. The proposed approach leverages both verbal and encouragement feedbacks from the teacher for joint learning, thus overcoming the difficulties encountered with either only  imitation or reinforcement.

Leveraging jointly imitation and reinforcement is crucial.
On the one hand, the agent trained by pure imitation is not necessarily able to converse adaptively within context due to the negligence of the reinforcement signal.
An example is that it is hard to make a successful conversation with a well-trained parrot, which is only good at mimicking.
The reason is that the learner is mimicking from a third person perspective,  mimicking the teacher who is conversing with it, thus certain words in the sentences from the teacher such as ``\emph{yes/no}'' and ``\emph{you/I}'' might need to be removed/adapted due to the change of perspective from teacher to learner. 
On the other hand, it is also challenging to generate appropriate conversational actions using purely the reinforcement signal without imitation, due to the inability of speaking, thus the probability of generating a sensible sentence by randomly uttering is low, let alone that of a proper one.
This is exemplified by the fact that babies don't fully develop their language capabilities without the ability to hear, which is one of the most important channels for language-related imitation.

【Example】show the process 


%This work presents an interactive setting for grounded natural language learning, where an agent learns natural language by interacting with a teacher and learning from feedback, thus learning and improving language skills while taking part in the conversation.
%
%Inspired by the way We further present a grounded natural language learning approach under the interactive setting  by leveraging feedbacks from the teacher during interaction through joint imitation and reinforcement.

Results
The end result is that the agent learns to converse with teacher properly by purely interacting with teacher, starting from the stage of knowing nothing about natural language.
Our agent also has desirable generalization and transferring abilities under several different scenarios

[another example]




Next step
This work is our initial exploration in the direction of interaction-based language learning. Initial language learning ability has been shown in the current simple setting.
Our next step includes increasing the complexity of the language learning environment.

As for future work, we would like to explore the direction of explicit modeling of learned knowledge and fast learning about new concepts.
Another interesting direction is to connect the language learning task presented in this paper with other heterogeneous tasks such as navigation.





